The design and performance of an improved target for MICE

The linear motor driving the target for the Muon Ionisation Cooling Experiment has been redesigned to improve its reliability and performance. A new coil-winding technique is described which produces better magnetic alignment and improves heat transport out of the windings. Improved field-mapping has allowed the more precise construction to be demonstrated, and an enhanced controller exploits the full features of the hardware, enabling increased acceleration and precision. The new user interface is described and analysis of performance data to monitor friction is shown to allow quality control of bearings and a measure of the ageing of targets during use.

==> 02-Stator/02-04-Inductance.tex <==
%
%--------  Stator: Inductance
\subsection{Inductance and resistance measurements}
\label{Sect:Stator:Inductance}
%
Who was going to write this?
Is it required?
Inductance measurement is included in 2.1.



==> 03-Shaft/03-Shaft.tex <==
%
%--------  Shaft
\section{Target shaft}
\label{Sect:Shaft}

This section to be written by Jason.





==> styles/TargetPaper_def.tex <==
%------------------------------------------------------------------------------
% New command definitions, constants, etc. for the Physics Group contribution
%                               to the ISS report
% ===========================================================================
%
%  History:
%    KL: 07Feb06: First version
%    KL: 21Aug06: Remove \eq (commented)
%    KL: 10Sep06: Add \GeV, \eV
%    KL: 05Jun07: Hyphenation options added.
%------------------------------------------------------------------------------
%	Some special symbols etc.:
%       --------------------------
%       -> small numbers
%------------------------------------------------------------------------------
\def\zero{{\scriptscriptstyle 0}}
\def\sone{{\scriptscriptstyle 1}}
\def\stwo{{\scriptscriptstyle 2}}
\def\sthr{{\scriptscriptstyle 3}}
\def\sfou{{\scriptscriptstyle 4}}
\def\sfiv{{\scriptscriptstyle 5}}
\def\sfiv{{\scriptscriptstyle 5}}
\def\ssix{{\scriptscriptstyle 6}}
\def\ssev{{\scriptscriptstyle 7}}
\def\seig{{\scriptscriptstyle 8}}
\def\snin{{\scriptscriptstyle 9}}
\def\sten{{\scriptscriptstyle 10}}
\def\half{{\scriptscriptstyle 1/2}}
%------------------------------------------------------------------------------
%       -> eV and multiples
%------------------------------------------------------------------------------
\def\Ev{\ensuremath{\text{e}\text{V\/}}}
\def\eV{\ensuremath{\text{e}\text{V\/}}}
\def\Kev{\ensuremath{\text{ke}\text{V\/}}}
\def\Mev{\ensuremath{\text{Me}\text{V\/}}}
\def\Gev{\ensuremath{\text{Ge}\text{V\/}}}
\def\GeV{\ensuremath{\text{Ge}\text{V\/}}}
\def\Gevc{\ensuremath{\text{Ge}\text{V\/}/c}}
\def\Gevcs{\ensuremath{\text{Ge}\text{V\/}/c^2}}
\def\Tev{\ensuremath{\text{Te}\text{V\/}}}
\def\ev{\ensuremath{\,\text{e}\text{V\/}}}
\def\kev{\ensuremath{\,\text{ke}\text{V\/}}}
\def\mev{\ensuremath{\,\text{Me}\text{V\/}}}
\def\gev{\ensuremath{\,\text{Ge}\text{V\/}}}
\def\gevc{\ensuremath{\,\text{Ge}\text{V\/}/c}}
\def\gevcs{\ensuremath{\,\text{Ge}\text{V\/}/c^2}}
\def\tev{\ensuremath{\,\text{Te}\text{V\/}}}
%------------------------------------------------------------------------------
%       -> various other units (for math mode only)
%------------------------------------------------------------------------------
\def\pb{\,\text{pb}}
\def\fb{\,\text{fb}}
\def\pbi{\,\text{pb}^{-1}}
\def\m{\,\text{m}}
\def\cm{\,\text{cm}}
\def\mm{\,\text{mm}}
\def\km{\,\text{km}}
\def\mum{\,\mu\text{m}}
\def\mA{\,\text{mA}}
\def\Hz{\,\text{Hz}}
\def\kHz{\,\text{kHz}}
\def\MHz{\,\text{MHz}}
\def\ppm{\,\text{ppm}}
\def\scnd{\,\text{s}}
\def\musec{\,\mu\text{s}}
\def\ns{\,\text{ns}}
\def\rad{\,\text{rad}}
\def\mrad{\,\text{mrad}}
\def\murad{\,\mu\text{rad}}
%------------------------------------------------------------------------------
%       -> commonly used symbols
%------------------------------------------------------------------------------
\def\BR{{\rm BR}}
\def\CC{{\scriptscriptstyle{\rm CC}}}
\def\CI{{\scriptscriptstyle{\rm CI}}}
\def\DA{{\scriptscriptstyle{\rm DA}}}
\def\DO{{D{\O}}\xspace}
\def\DCA{{\rm DCA}}
\def\F{{\cal F}}
\def\GRV{{\scriptscriptstyle{\rm GRV}}}
\def\IC{{\scriptscriptstyle{\rm IC}}}
\def\ISR{{\scriptscriptstyle{\rm ISR}}}
\def\IP{{\rm I$@,$P}}
\def\JB{{\scriptscriptstyle{\rm JB}}}
\def\L{{\scriptscriptstyle{\rm L}}}
\def\LL{{\scriptscriptstyle{\rm LL}}}
\def\LQbar{\overline{\rm LQ}}
\def\LQsub{{\scriptscriptstyle{\rm LQ}}}
\def\LQ{{\rm LQ}}
\def\LR{{\scriptscriptstyle{\rm LR}}}
\def\Ldes{{\cal L}_{\rm des}}
\def\Lumi{{\cal L}}
\def\MC{{\scriptscriptstyle{\rm MC}}}
\def\MSbar{\hbox{$\overline{\rm MS}$}}
\def\NC{{\scriptscriptstyle{\rm NC}}}
\def\NS{{\scriptscriptstyle{\rm NS}}}
\def\Prob{{\cal P}}
\def\QPM{{\scriptscriptstyle{\rm QPM}}}
\def\RL{{\scriptscriptstyle{\rm RL}}}
\def\RPv{{{\not R}_P}}
\def\RR{{\scriptscriptstyle{\rm RR}}}
\def\R{{\scriptscriptstyle{\rm R}}}
\def\SM{{\scriptscriptstyle{\rm SM}}}
\def\SU2U1{{\rm SU}(2)\times{\rm U}(1)}
\def\Ssup{{\scriptscriptstyle{\rm S}}}
\def\XXX{\hbox{\bf ??}}
\def\alsmu#1{{\alpha_s(\mu_{#1}^2)}}
\def\alsmz{{\alpha_s(M_Z^2)}}
\def\alsqs{{\alpha_s(Q^2)}}
\def\als{{\alpha_s}}
\def\ctwb{\cos\theta_{\scriptscriptstyle W}}
\def\ctws{\cos^2\theta_{\scriptscriptstyle W}}
\def\cut{{\rm cut}}
\def\data{{\rm data}}
\def\det{{\rm det}}
\def\dof{{\rm dof}}
\def\elm{{\rm elm}}
\def\epslam{{\epsilon/\Lambda^2}}
\def\exc{{\rm exc}}
\def\exp{{\rm exp}}
\def\gh{{\gamma_h}}
\def\had{{\rm had}}
\def\kg{{k_\gamma}}
\def\lsq#1{{\lambda_{#1}}}
\def\lsqp#1{{\lambda'_{#1}}}
\def\lsqpp#1{{{\lambda''}_{#1}}}
\def\max{{\rm max}}
\def\meas{{\rm meas}}
\def\min{{\rm min}}
\def\obs{{\rm obs}}
\def\ord#1{{\cal O}(#1)}
\def\rnge{{\,\text{--}\,}}
\def\sca{{\rm sca}}
\def\sihat{{\hat\sigma}}
\def\slim{{\rm lim}}
\def\slimb{{\rm lim,B}}
\def\slimr{{\rm lim,R}}
\def\smin{{\rm min}}
\def\smax{{\rm max}}
\def\stwb{\sin\theta_{\scriptscriptstyle W}}
\def\stwss{\sin^4\theta_{\scriptscriptstyle W}}
\def\stws{\sin^2\theta_{\scriptscriptstyle W}}
\def\sys{{\rm sys}}
\def\ta{{\theta^\ast}}
\def\tilR{\tilde R}
\def\tilS{\tilde S}
\def\tilU{\tilde U}
\def\tilV{\tilde V}
\def\tl{{\theta_\ell}}
\def\tot{{\rm tot}}
\def\true{{\rm true}}
\def\tw{\theta_{\scriptscriptstyle W}}
%------------------------------------------------------------------------------
%       -> some math symbols (+,-,...) for usage as mathchar's
%------------------------------------------------------------------------------
\mathchardef\qsm=63
\mathchardef\pls=43
\mathchardef\mns=512
\mathchardef\plm=518
\mathchardef\eql=61
\mathchardef\smallleft=300
\mathchardef\smallright=301
\mathchardef\perslsh=47
\mathchardef\les=316
\mathchardef\gre=318
\mathchardef\leq=532
\mathchardef\grq=533
%------------------------------------------------------------------------------
%       -> characters for typewriter font (used for http addresses)
%------------------------------------------------------------------------------
\chardef\usc=95
\chardef\til=126
%------------------------------------------------------------------------------
%       -> shorthand for "integral limits below and above"
%------------------------------------------------------------------------------
\def\intl{\int\limits}
%------------------------------------------------------------------------------
%       -> footenote markers
%------------------------------------------------------------------------------
\def\fdag{$^{{\displaystyle\dagger})}$}
\def\fddag{$^{{\displaystyle\ddagger})}$}
\def\fstar{$^{{\displaystyle\star})}$}
\def\faste{$^{{\displaystyle\ast})}$}
%------------------------------------------------------------------------------
%       -> d'Alembert operator
%------------------------------------------------------------------------------
\def\sqr#1#2#3{{\vcenter{\hrule height.#3ex\hbox{\vrule width.#2ex height#1ex
    \kern#1ex\vrule width.#3ex}\hrule height.#2ex}}}
\def\dalem{\mathchoice\sqr{1.6}{08}{24}\sqr{1.6}{08}{24}
                      \sqr{1.4}{07}{21}\sqr{1.1}{06}{18}}
%------------------------------------------------------------------------------
%       -> rectangle with arrow ( '-> )
%------------------------------------------------------------------------------
\def\angleto{\vrule width.035em height2.1ex depth-.56ex\unskip\kern-.6ex\to}
%------------------------------------------------------------------------------
%       -> permille sign
%------------------------------------------------------------------------------
\def\perchc#1{{\raise.4ex\hbox{$\mkern4mu#1{\it\perslsh}_
             {\mkern-5mu\scriptscriptstyle{{\rm o}\!{\rm o}}}^
             {\mkern-12.8mu\scriptscriptstyle{\rm o}}$}}}
\def\permil{{\mathchoice\perchc{\displaystyle}\perchc{\textstyle}
             \perchc{\scriptstyle}\perchc{\scriptscriptstyle}}}
%------------------------------------------------------------------------------
%       -> wide bar and bar in parantheses as mathaccents, some applications
%------------------------------------------------------------------------------
\def\widebar#1{\mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.mu}\mkern1.mu}
\catcode`\@=11 % @ signs are now treated as letters
\def\parenbar{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}
\catcode`\@=12 % @ signs are no longer letters
\def\nuan{\ensuremath{\parenbar{\nu}}}
\def\qqbar{\ensuremath{\parenbar{q}}}
\def\pbar{\ensuremath{\widebar{p}}}
\def\qbar{\ensuremath{\widebar{q}}}
\def\dbar{\ensuremath{\widebar{d}}}
\def\ubar{\ensuremath{\widebar{u}}}
\def\sbar{\ensuremath{\widebar{s}}}
\def\cbar{\ensuremath{\widebar{c}}}
\def\bbar{\ensuremath{\widebar{b}}}
\def\tbar{\ensuremath{\widebar{t}}}
\def\nubar{\ensuremath{\widebar{\nu}}}
\def\Dbar{\ensuremath{\widebar{D}}}
\def\ebar{\ensuremath{\widebar{e}}}
%------------------------------------------------------------------------------
%	Some shorthands and utilities:
%       ------------------------------
%       -> vertical rule of width zero and variable height & depth
%------------------------------------------------------------------------------
\newbox\struttbox
\setbox\struttbox=\hbox{\vrule height1.65ex depth.485ex width0pt}
\def\strutt{\relax\ifmmode\copy\struttbox\else\unhcopy\struttbox\fi}
\def\stru#1#2{\relax\ifmmode\hbox{\vrule height#1 depth#2 width0pt}
\else\vrule height#1 depth#2 width0pt\fi}
%------------------------------------------------------------------------------
%       -> underline with resonable distance text - line
%------------------------------------------------------------------------------
\def\uline#1{$\underline{\hbox{#1\strutt}}$}
%------------------------------------------------------------------------------
%       -> roman numbers (uppercase and lowercase)
%------------------------------------------------------------------------------
\def\ronum#1{\uppercase\expandafter{\romannumeral#1}}
\def\ronuml#1{\expandafter{\romannumeral#1}}
%------------------------------------------------------------------------------
%       -> vectors and matrices
%------------------------------------------------------------------------------
\def\vect#1{\begin{matrix}#1\end{matrix}}
\def\pvect#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bvect#1{\begin{bmatrix}#1\end{bmatrix}}
%------------------------------------------------------------------------------
%       -> some alignment tools for tables
%------------------------------------------------------------------------------
\def\cA{{\phantom{0}}}
\def\cB{{\phantom{00}}}
\def\cC{{\phantom{000}}}
\def\cD{{\phantom{0000}}}
\def\cM{{\phantom{\mns}}}
%------------------------------------------------------------------------------
%       -> shorthand for protected citations in captions
%------------------------------------------------------------------------------
\def\pcite#1{\protect\cite{#1}}
%------------------------------------------------------------------------------
%       -> shorthands for equation, figure, table, section references
%------------------------------------------------------------------------------
%\def\eq#1{eq.~(\ref{eq-#1})}
\def\eqsand#1#2{eqs.~(\ref{eq-#1}) and~(\ref{eq-#2})}
\def\eqsto#1#2{eqs.~(\ref{eq-#1}-\ref{eq-#2})}
\def\eqstwo#1#2{eqs.~(\ref{eq-#1},\ref{eq-#2})}
\def\eqsthr#1#2#3{eqs.~(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3})}
\def\eqsfou#1#2#3#4{eqs.~(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3},\ref{eq-#4})}
\def\Eq#1{Equation~(\ref{eq-#1})}
\def\Eqsto#1#2{Equations~(\ref{eq-#1}-\ref{eq-#2})}
%\def\fig#1{Fig.~\ref{fig-#1}}
\def\figs#1{Fig.~\ref{fig-#1}}
\def\Fig#1{Figure~\ref{fig-#1}}
\def\figand#1#2{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\def\figand#1#2{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\def\tab#1{Table~\ref{tab-#1}}
\def\tabsand#1#2{Tables~\ref{tab-#1} and~\ref{tab-#2}}
\def\Tab#1{Table~\ref{tab-#1}}
\def\sec#1{Sect.~\ref{sec-#1}}
\def\Sec#1{Section~\ref{sec-#1}}
\def\secand#1#2{Sects.~\ref{sec-#1} and~\ref{sec-#2}}
\def\secsto#1#2{Sects.\ref{sec-#1} to~\ref{sec-#2}}
%------------------------------------------------------------------------------
%	Local laguage changes
%       ---------------------
%------------------------------------------------------------------------------
\def\german#1{\selectlanguage{german}#1\selectlanguage{english}}
%------------------------------------------------------------------------------
%	Redefine mathbf
%       ---------------
%------------------------------------------------------------------------------
%\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{sl}
\def\mb{\mathbf}
%------------------------------------------------------------------------------
%
% New commands:
%
%------------------------------------------------------------------------------
%
\newcommand{\address}{ } 
%
\newcommand{\gevsq}     {\mbox{${\rm GeV}^2$}}
\newcommand{\qsd}       {\mbox{${Q^2}$}}
\newcommand{\PTM}       {P_{T\rm miss}}
\newcommand{\x}         {\mbox{${\it x}$}}
\newcommand{\y}         {\mbox{${\it y}$}}
\newcommand{\ye}        {\mbox{${y_{e}}$}}
\newcommand{\smallqsd}  {\mbox{${q^2}$}}
\newcommand{\rambox}    {\mbox{$ \rightarrow $}}
\newcommand{\ra}        {$\rightarrow$}
\newcommand{\ygen}      {\mbox{${y_{gen}}$}}
\newcommand{\yjb}       {\mbox{${y_{_{JB}}}$}}
\newcommand{\yda}       {\mbox{${y_{_{DA}}}$}}
\newcommand{\qda}       {\mbox{${Q^2_{_{DA}}}$}}
\newcommand{\qjb}       {\mbox{${Q^2_{_{JB}}}$}}
\newcommand{\ypt}       {\mbox{${y_{_{PT}}}$}}
\newcommand{\qpt}       {\mbox{${Q^2_{_{PT}}}$}}
\newcommand{\ypr}       {\mbox{${y_{(1)}}$}}
\newcommand{\yprpr}     {\mbox{${y_{(2)}}$}}
\newcommand{\ypps}      {\mbox{${y_{(2)}^2}$}}
\newcommand{\gammah}    {\mbox{$\gamma_{_{H}}$}}
\newcommand{\gammahc}   {\mbox{$\gamma_{_{PT}}$}}
\newcommand{\gap}       {\hspace{0.5cm}}
\newcommand{\gsim}      {\mbox{\raisebox{-0.4ex}{$\;\stackrel{>}{\scriptstyle \sim}\;$}}}
\newcommand{\lsim}      {\mbox{\raisebox{-0.4ex}{$\;\stackrel{<}{\scriptstyle \sim}\;$}}}
\renewcommand{\thefootnote}{\arabic{footnote}}
%
%----------------------------------------------------------------------------
%
% Constants etc.
% ==============
%
%----------------------------------------------------------------------------
% Define (e.g.) working value of theta_23?
%
%----------------------------------------------------------------------------
%
% Paper format
% ============
%
%----------------------------------------------------------------------------
%
%------------------------------------------------------------------------------
%	page layout
%------------------------------------------------------------------------------
\paperheight    29.7cm
\paperwidth     21.0cm
%------------------------------------------------------------------------------
%	... horizontal spacings
%------------------------------------------------------------------------------
\textwidth      16.0cm
\evensidemargin -0.3cm
\oddsidemargin  -0.3cm
%------------------------------------------------------------------------------
%	... vertical spacings
%------------------------------------------------------------------------------
\textheight     650.pt
%\topmargin      -1.5cm -- KL 18Apr06
\footskip        1.0cm
%------------------------------------------------------------------------------
%	interline spacing, paragraph indention etc.
%------------------------------------------------------------------------------
\renewcommand{\baselinestretch}{1.12}
\renewcommand{\arraystretch}{1.1}
\parindent       0.0pt
\parskip         0.3cm plus0.05cm minus0.05cm
\overfullrule    0.0pt
%------------------------------------------------------------------------------
%	item spacings
%------------------------------------------------------------------------------
\itemsep    0.2ex plus 0.1ex minus 0.15ex
\topsep     0.2ex plus 0.1ex minus 0.15ex
\partopsep  1.2ex plus 0.6ex minus 0.6ex
\setlength\leftmargini   {1.6em}
\setlength\leftmarginii  {1.4em}
\setlength\leftmarginiii {1.2em}
\setlength\leftmarginiv  {1.0em}
%------------------------------------------------------------------------------
%	"tight item" environments
%------------------------------------------------------------------------------
\newenvironment{tightitemize}[2]
 {\begin{list}{$\bullet$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
\newenvironment{tightsubitemize}[2]
 {\begin{list}{$-$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
\newenvironment{tightssubitemize}[2]
 {\begin{list}{$\to$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
%------------------------------------------------------------------------------
%	float parameters
%------------------------------------------------------------------------------
\renewcommand{\topfraction}{1.}
\renewcommand{\bottomfraction}{1.}
\renewcommand{\textfraction}{0.01}
\setlength{\floatsep}{6pt plus 3pt minus 3pt}
\setlength{\textfloatsep}{12pt plus 8pt minus 4pt}
%------------------------------------------------------------------------------
%	adjust footnote design
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newlength{\@fninsert}
\setlength{\@fninsert}{0.6em}
\newlength{\@fnwidth}
\setlength{\@fnwidth}{\textwidth}
\addtolength{\@fnwidth}{-\@fninsert}
\addtolength{\@fnwidth}{-0.4em}
\renewcommand{\@makefntext}[1]%
  {\noindent\makebox[\@fninsert][r]{\@makefnmark}\hfil%
  \parbox[t]{\@fnwidth}{#1}}
\catcode`\@=12 % @ signs are no longer letters
\addtolength{\skip\footins}{2.mm}
%------------------------------------------------------------------------------
%	equation numbers like (n.k): n=section, k=equation
%------------------------------------------------------------------------------
%\numberwithin{equation}{section}
%\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
%------------------------------------------------------------------------------
%	set section numbering depth (5: allow for sections up to i.j.k.l.m.)
%       and redefine section, subsection, subsubsection, paragraph 
%       to yield a proper heading
%       force four levels of headers in the table of contents
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\setcounter{secnumdepth}{5}
\setcounter{tocdepth}{4}
\renewcommand\section{\@startsection{section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalfont\Large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-3.25ex\@plus -1ex \@minus -.2ex}%
                                   {1.5ex \@plus .2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {-3.25ex\@plus -1ex \@minus -.2ex}%
                                   {1.5ex \@plus .2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {3.25ex \@plus1ex \@minus.2ex}%
                                   {1.2ex \@plus .2ex}%
                                   {\normalfont\normalsize\bfseries}}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%	separators for subsections and sections
%------------------------------------------------------------------------------
\def\sectionsep{\strut}
\def\chaptersep{\vfill\eject}
%------------------------------------------------------------------------------
%	Add hyphenation options
%------------------------------------------------------------------------------
\hyphenation{par-ti-cu-lar} \hyphenation{ex-pe-ri-men-tal}
\hyphenation{dif-fe-rent} \hyphenation{bet-we-en}
\hyphenation{mo-du-lus}
%
%--------  End  --------  --------  --------  --------  --------  --------

